Understanding the Effect of Bias in Deep Anomaly Detection

Anomaly detection presents a unique challenge in machine learning, due to the scarcity of labeled anomaly data. Recent work attempts to mitigate such problems by augmenting training of deep anomaly detection models with additional labeled anomaly samples. However, the labeled data often does not align with the target distribution and introduces harmful bias to the trained model. In this paper, we aim to understand the effect of a biased anomaly set on anomaly detection. Concretely, we view anomaly detection as a supervised learning task where the objective is to optimize the recall at a given false positive rate. We formally study the relative scoring bias of an anomaly detector, defined as the difference in performance with respect to a baseline anomaly detector. We establish the first finite sample rates for estimating the relative scoring bias for deep anomaly detection, and empirically validate our theoretical results on both synthetic and real-world datasets. We also provide an extensive empirical study on how a biased training anomaly set affects the anomaly score function and therefore the detection performance on different anomaly classes. Our study demonstrates scenarios in which the biased anomaly set can be useful or problematic, and provides a solid benchmark for future research.

==> 1-intro.tex <==
% !TEX root =  main.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ziyu{The following is the original version without the bayes optimal unbiased detector part. The story version with bayes optimal unbiased detector is currently in Section 3 (main story \& side story).}

We are motivated by this couter-intuitive phenomenon: semi-supervised models can perform much worse than unsupervised models. We would like to understand this phenomenon, and we achieve this by the following two-step approaches with one hypothesis.

\textbf{Hypothesis}. \quad We assume that the difference in model performance comes from scoring bias. Given any two models, the scores assigned by them on a data point has a certain score difference ($\delta(x)=s(x)-\tilde{s}(x)$). Formally, our hypothesis throughout the paper is that: given a data distribution, the aforementioned scoring bias (defined on two models / scoring function) would follow a distribution. \todo{make hypothesis on scores instead of score difference; scoring bias referring to $\xi$ as the performance difference}.

Based on this hypothesis, our paper is organized as the following two parts: (1) theory part: given two score functions, how to estimate and guarantee the resulting performance change; (2) analysis part: for a specific model pair (i.e. unsupervised model v.s. supervised model), how to estimate their scoring bias for different data distribution. (\todo{3 sets of figures: 1. umap embeddings; 2. score bias distributions; 3. detection rates}).

% Section 3: formally define bias
% Section 4: define the test time bias (?)


In section 3, we formally introduce the notion of bias in the context of anomaly detection. 

In section 4, test time, 

In section 5, we show that, perhaps surprisingly, training


\textbf{Part 1: Theory}. \quad As stated above, here we will be answering two questions:
\begin{itemize}
    \item Knowing the scoring bias on a data distribution of two models follows a distribution, can we know the performance difference of the two models? \todo{p.s. Remember to add the performance metric in section 3 or so, and we need to mention that both fixed fpr strategy and fixed recall strategy works and we just choose one of them. (But will we be asked why not f1?)}
    \item Theoretically, could we guarantee the empirical performance difference would converge to the theoretical performance difference we estimated in question 1?
\end{itemize}
For the first question, we provide a simple formula from scoring bias to performance bias; specifically, assuming the scoring bias is of normal distribution, there exists an analytical form of this formula (p.s. note that we here also additionally assumed that score distribution itself also follows the normal distribution). For the second question, we provide a rigorous theoretical bound, i.e. a finite sample convergence rate. As long as the sample complexity reaches the bound we proposed, the performance difference should converge to the value we have calculated.

Overall, this part is embodied in Section 4. It guarantees the performance change that we can observe under certain scoring bias. Only with this theory in hand, we could be able to confidently say that the performance change is guaranteed, instead of an unstable fluctuation. (Note that all this depends on our hypothesis on the scoring bias, which may not be used in our second version of story with optimal bayes detector).

\textbf{Part 2: Analysis}. The previous part bridges "performance change" with "scoring bias". In this part, we want to understand or interpret where does scoring bias come from. As stated above, we want to answer this question: for a specific model pair (i.e. unsupervised model v.s. supervised model), how to estimate their scoring bias for different data distribution. Here we would first present experiment results, then summarize them to be 2 or 3 hypotheses.


\textbf{Loophole for this current version.} 
\begin{itemize}
    \item The difference of two models does not have theoretical importance, they only have practical usage (i.e. to determine which model to use). In traditional ML literature, it is more common to use bias to describe the performance difference to the optimal model.
    \item Also, for section 5, if we do not have a clearly defined "bias", it would be hard to provide a general hypothesis or rule to explain for the performance difference between unsupervised model and semi-supervised model, whether on the trained type of abnormal data or the untrained ones. If we have the definition or theory of optimal detector, it would be naturally described (see the $D_{m, i}$ and $D_{m, j}$ part in Section 3.2.)
\end{itemize}



\ziyu{The following texts (from here up to section 2) are old texts and are mostly useless.}

(Backgrounds) We are motivated by the phenomenon that sometimes additional abnormal data in training can bring adverse effect to detect anomaly data in testing. This is an critical but often ignored issue which can have huge impact in many real-world practice. To figure out the reason and provide a better training protocol, we must first understand the mechanism for training with additional abnormal data, \textit{i.e.}, semi-supervised anomaly detection.

\todo{Modify the motivation, maybe less semi-supervised concentrated? The scoring bias in both data and training procedures. Or maybe we can say "modern anomaly detection" approaches, which usually incorporates additional labeled abnormal data?}

We decompose this problem into two sub-problems.

\todo{We need a formal description for \textbf{scoring bias}.}

Section 4 is on the valiation of the performance of an anomaly detection model. More specifically, (1) scoring bias exists for anomaly detection models (for both unsupervised and semi-supervised ones). (2) Knowing the measure (magnitude) of the scoring bias, can we know the resulting detection performance? (i.e. $\xi$ as a function of $\delta (\cdot)$) (3) If so, how much and by what means can we guarantee the performance? (The answer is by sample complexity.)

There remains an unanswered question in Section 4 – the sources of scoring bias. In Section 4, we acts in an \textit{ex post} way: knwoing empirical CDFs, estimating the $\xi$ (performance change introduced by bias) by fitting a distribution to empirical CDFs, and evaluating the correctness for resulting performance.

However, in practice, we need an \textit{ex ante} way, that is to estimate $\xi$ before training (and knowing the empirical CDF). This is helpful as it reveals the uncertainties (vulnerabilities and strenghs) of current model. It can in turn help us to improve the model.

To achieve this this, we want an approximate function from the knowns (model and data) to scoring bias (i.e. $\delta (\cdot)$ as a function of $D_{train}$, $D_{test}$ and the model $\phi (\cdot)$). More specifically, knowing information of the trained data and test data (e.g. their triplet divergence, conditional mutual info, etc.), we want to estimate the $\mu$ and $\sigma$ for the distribution (Guassian fitted) of $\delta (\cdot)$.


% Firstly, we assume that additional abnormal data in training will impose a bias on the anomaly scoring function by model; under this assumption, we derive the performance guarantee for semi-supervised anomaly detection models. Namely, the first problem we are studying is – what the detection rate of the model will be, assuming there is a anomaly scoring bias on the model.

% Secondly, we attempt to validate and instantiate the assumption of anomaly scoring bias. We will try to characterize the cause of the scoring bias from the perspective from model and data respectively.

Combining the two, we would be able to provide a rigorous theoretical analysis for the performance of modern anomaly detection (i.e. by modern we refer to semi-supervised training with additional labeled anomalies). For next steps, we may be able to, in theory: (1) make the above theory more rigorous by a Bayes framework: considering the \textit{ex ante} estimate as prior and the \textit{ex post} estimate as posterior, (2) (combining with transfer learning), extend to classification problems, specifically on recently hot self-supervised training protocol; and in practice: (1) construct an adaptive learning framework for more confident and evolving anomaly detection models.



% Baseline model can achieve a target recall.
% A new data distribution / model improve the performance up a certain margin, \xi.
% The recall rate r0 for the baseline model is accurate, the empirical recall rate for our method is w.h.p. at least r0 + xi.

% polluted S_0

% in section 4, score function is stable, or even deterministic

\textbf{Original Story}. 
\begin{itemize}
    \item Assuming there exists scoring bias for different models. \todo{Need to address the existence of scoring bias.}
\end{itemize}

\todo{Section 4 need to formally propose the performance metric.}

Dependent on if we could give an unbiased algorithm, we may need to change the name of "scoring bias" or "relative scoring bias".
(Remark: maximize recall can also achieved)



==> 2-lit-old.tex <==
% !TEX root =  main.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Related Work}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \vspace{-6pt}
\para{Anomaly Detection Models.} \rebuttal{While the literature on anomaly detection models is extensive, the most relevant to our work are deep learning based models.
%unsupervised and semi-supervised anomaly detection models.
Following the terminology used by~\cite{anormaly-survey-2009}, we consider two types of models: \vspace{-0.06in}
\begin{packed_itemize}
\item {\em Semi-supervised anomaly detection} refers to models trained on only normal data, e.g., ~\cite{pmlr-v80-ruff18a,ADae,Zhou2017AE};
\item {\em Supervised anomaly detection} refers to models trained on  normal data and a small set of labeled anomalies, e.g.,~\cite{pang2019deep, daniel2019deep, yamanaka2019autoencoding, ruff2020rethinking,ruff2020deep}.\vspace{-0.06in}
\end{packed_itemize}
}
One can also categorize models by their architecture: hypersphere~\citep{pmlr-v80-ruff18a,ruff2020rethinking,ruff2020deep} and autoencoder (or reconstruction) based models~\citep{Zhou2017AE,yamanaka2019autoencoding}.

%\footnote{We note that a set of works refer to this type of models as unsupervised anomaly detection %models, while others term them as semi-supervised models~\citep{anormaly-survey-2009}.  In this work, %we refer to them as the baseline semi-supervised models.}


Another line of recent work proposes to use synthetic or auxiliary anomalies to train anomaly detection models (\cite{golan2018deep, hendrycks2019using, lee2018training, hendrycks2019oe}), ``forcing'' the model to learn a more compact representation of the normal data. While the existing work has shown empirically that the choice of abnormal data in training can help detect some unseen abnormal distributions, it does not offer any theoretical explanation for the phenomenon, nor does it consider the counter-cases when additional abnormal data in training hurt the detection performance.

\para{Bias in Anomaly Detection.} To the best of our knowledge, we are the first to identify the presence of bias caused by an additional labeled anomaly set in deep anomaly detection models, especially when there exists a mismatch between the anomalies present in training and those encountered in testing (as shown in Section~\ref{sec:eval}). Existing work has explored the presence of bias in \rebuttal{semi-supervised} anomaly detection models when there exists defective {\em normal} data in training, like outliers and simple-to-reconstruct examples \citep{tong2019fixing}, or examples with background noise \citep{liu2019exploring}. There is also literature on the bias-variance tradeoff for ensembles of semi-supervised anomaly detection models \citep{aggarwal2015theoretical, rayana2016sequential}.  But little or no work has been done on the bias of anomaly detection in the supervised setting \rebuttal{(i.e., models trained on both normal data and some labeled anomalies)}.  Finally, another line of work in transfer learning has identified the value of additional labeled data in training \citep{kpotufe2018marginal, hanneke2019value} and the performance bias on target data by transferring knowledge from a less related source \citep{wang2019characterizing, wu2020understanding}.  Yet most work only considered the cases of classification models.

\para{PAC guarantees for Anomaly Detection.} Despite significant progress on developing theoretical guarantees for classification tasks (\cite{valiant1984theory, kearns1994introduction}), little has been done for anomaly detection tasks. \cite{siddiqui2016finite} first establishes a PAC framework for anomaly detection models using the notion of pattern space; however, it is hard to apply such pattern spaces  to deep learning models with complex latent spaces. \cite{liu2018open} proposes a model-agnostic approach to provide the PAC guarantee for anomaly detection performance,  by analyzing the convergence for the cumulative distribution of anomaly scores. We follow the basic setting from this line of work to address the convergence of the relative scoring bias. In contrast to prior work, our proof relies on a novel adaption of the key theoretical tool from \cite{massart1990}, which allows us to extend our theory to characterize the notion of scoring bias as defined in Section~\ref{sec:defbias}.
%addition to the key In addition to the  We follow this line of work to establish our theory in the presence of relative scoring bias. \todo{how do we differ from Liu}


==> macros.tex <==
% !TEX root =  main.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% if you need to pass options to natbib, use, e.g.:
%     \PassOptionsToPackage{numbers, compress}{natbib}
% before loading neurips_2020

% ready for submission
% \usepackage{neurips_2020}

% to compile a preprint version, e.g., for submission to arXiv, add add the
% [preprint] option:
%     \usepackage[preprint]{neurips_2020}

% to compile a camera-ready version, add the [final] option, e.g.:
%     \usepackage[final]{neurips_2020}

% to avoid loading the natbib package, add option nonatbib:
     \usepackage[nonatbib]{iclr2021_conference}

% Attempt to make hyperref and algorithmic work together better:
\newcommand{\theHalgorithm}{\arabic{algorithm}}
%\usepackage{algorithm}
%\usepackage{algorithmic}


%\usepackage{times}
\usepackage{savesym,multirow,url,xspace,graphicx,hyperref,enumitem,color}
\usepackage[dvipsnames]{xcolor}
\usepackage[titletoc]{appendix}
%\usepackage[tight]{subfigure}
\usepackage{subcaption}
\usepackage{dsfont}
\usepackage{multicol}

% toggle command
\usepackage{etoolbox}
%----------------Macros from colt
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
%\usepackage[final]{neurips_2018}
\usepackage{tikz}
\usepackage{pgfplots}
\usepackage{verbatim}
\usepackage{amsmath,bm}
%\usepackage{algorithm}
\usepackage{multirow}
\usepackage{mathtools}
\usepackage{comment}
%\usepackage{algorithmicx}
%\usepackage[ruled]{algorithm}
%\usepackage{algorithmic}
%\usepackage[noend]{algpseudocode}

% algorithm2e package
%\usepackage[lined, boxed, ruled, commentsnumbered, noend]{algorithm2e}

\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
%\SetCommentSty{mycommfont}

\newcommand{\argmin}{\operatornamewithlimits{arg\,min}}
\newcommand{\eqdef}{=\mathrel{\mathop:}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newtoggle{showcomments}
\settoggle{showcomments}{true}


%\newcommand{\val}{{\text{val}}}
%\newcommand{\citet}[1]{\citeauthor{#1} (\citeyear{#1})}
\iftoggle{showcomments}{
\newcommand{\annotate}[1]{{\textcolor{blue}{[{\bf Note:} #1]}}}
}
{
\newcommand{\annotate}[1]{}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newtoggle{longversion}
\settoggle{longversion}{true}

%\iftoggle{longversion}{\ref{app:sec..}}{Appendix E}.

% % toggle command
% \usepackage{etoolbox}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\newif\if@restonecol
\makeatother
\let\algorithm\relax
\let\endalgorithm\relax
\let\proof\relax
\let\endproof\relax
\usepackage[lined, boxed, ruled, commentsnumbered,noend]{algorithm2e}
%, noend
\usepackage{amsmath,amssymb,xfrac,amsthm}
\setitemize{noitemsep,topsep=1pt,parsep=1pt,partopsep=1pt, leftmargin=12pt}

%%%%%%%%%%%%%%%%%%%% OLD %%%%%%%%%%%%%%%%
\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}
\newtheorem*{theorem*}{Theorem}
\newtheorem{fact}{Fact}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{definition}{Definition}
%\newtheorem{assumption}{Assumption}
\newtheorem{example}{Example}
%%%%%%%%%%%%%%%%%%%% NEW %%%%%%%%%%%%%%%%
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{theorem}{Theorem}[section]
%\theoremstyle{definition}
\newtheorem{defn}{Definition}[section]
\newtheorem{assumption}{Assumption}%[section]
%\newtheorem{condition}{Condition}
\newtheorem{condition}[theorem]{Condition}

%\newtheorem{corollary}{Corollary}[theorem]
%\newtheorem{lemma}[theorem]{Lemma}




\makeatletter
\newcommand{\rmnum}[1]{\romannumeral #1}
\newcommand{\Rmnum}[1]{\expandafter\@slowromancap\romannumeral #1@}
%\usepackage{mathtools}
\makeatother
\usepackage{caption}
\newcounter{copyrightbox}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\denselist}{
  % \itemsep -2pt\topsep-8pt\partopsep-8pt
  \itemsep -2pt\topsep-5pt\partopsep-5pt\itemindent-10pt
}
\newcommand{\Rd}{\mathbb{R}^d}


% % References
% ----------------------------------------------------------------
\newcommand{\defref}[1]{Definition~\ref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}
\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\eqnref}[1]{\text{Eq.}~(\ref{#1})}
\newcommand{\secref}[1]{\S\ref{#1}}
\newcommand{\appref}[1]{Appendix \ref{#1}}
% \newcommand{\appref}[1]{the Appendix} % for short version of the paper
\newcommand{\thmref}[1]{Theorem~\ref{#1}}
\newcommand{\corref}[1]{Corollary~\ref{#1}}
\newcommand{\propref}[1]{Proposition~\ref{#1}}
\newcommand{\lemref}[1]{Lemma~\ref{#1}}
\newcommand{\conref}[1]{Condition~\ref{#1}}
\newcommand{\assref}[1]{Assumption~\ref{#1}}
%\newcommand{\algref}[1]{Algorithm~\ref{#1}}
\newcommand{\egref}[1]{Example~\ref{#1}}
\newcommand{\algoref}[1]{Algorithm~\ref{#1}}
%\newcommand{\lineref}[1]{Line~\ref{#1}}


% Text conveniences
% ------------------------------------------------------------------------------
\newcommand{\cf}{\emph{c.f.}}

% Wrappers: Parens, brackets, etc
% -------------------------------------------------------------------------------
\newcommand{\op}[1]{\operatorname{#1}}
\newcommand{\paren} [1] {\ensuremath{ \left( {#1} \right) }}
\newcommand{\parenb} [1] {\ensuremath{ \big( {#1} \big) }}
\newcommand{\bigparen} [1] {\ensuremath{ \Big( {#1} \Big) }}
\newcommand{\biggparen} [1] {\ensuremath{ \bigg( {#1} \bigg) }}
\newcommand{\Biggparen} [1] {\ensuremath{ \Bigg( {#1} \Bigg) }}
\newcommand{\bracket}[1]{\left[#1\right]}
\newcommand{\tuple}[1]{\ensuremath{\left\langle #1 \right\rangle}}
%\newcommand{\set}[1]{\ensuremath{\left\{#1\right\}}}
\newcommand{\curlybracket}[1]{\ensuremath{\left\{#1\right\}}}

\newcommand{\condcurlybracket}[2]{\ensuremath{\left\{#1\left\lvert\:#2\right.\right\}}}

% Functions and Functionals
% --------------------------------------------------------
\renewcommand{\Pr}[1]{\ensuremath{\mathbb{P}\left[#1\right] }}
\newcommand{\expct}[1]{\mathbb{E}\left[#1\right]}
\newcommand{\expctover}[2]{\mathbb{E}_{#1}\!\left[#2\right]}
%\newcommand{\E}[1]{\ensuremath{\mathbb{E}\left[#1\right] }}
\newcommand{\abs}[1]{\left\vert#1\right\vert}
%\newcommand{\argmax}{\operatorname{arg\,max}}
%\newcommand{\argmin}{\operatorname{arg\,min}}
\def \argmax {\mathop{\rm arg\,max}}
\def \argmin {\mathop{\rm arg\,min}}


% asymptotics
\newcommand{\littleO}[1]{\ensuremath{o\paren{#1}}}
\newcommand{\bigO}[1]{\ensuremath{\mathcal{O}\paren{#1}}}
\newcommand{\bigTheta}[1]{\ensuremath{\Theta\paren{#1}}}
\newcommand{\bigOmega}[1]{\ensuremath{\Omega\paren{#1}}}

\newcommand{\bigOTilde}[1]{\ensuremath{\tilde{O}\paren{#1}}}


% fundamental sets and objects
\newcommand{\NonNegativeReals}{\ensuremath{\mathbb{R}_{\ge 0}}}
\newcommand{\PositiveIntegers}{\ensuremath{\mathbb{Z^+}}}
\newcommand{\integers}{\ensuremath{\mathbb{Z}}}
\newcommand{\nats}{\ensuremath{\mathbb{N}}}
\newcommand{\reals}{\ensuremath{\mathbb{R}}}
\newcommand{\rationals}{\ensuremath{\mathbb{Q}}}
\newcommand{\distrib}[0]{\ensuremath{\mathcal{D}}}
\newcommand{\matroid}{\ensuremath{\mathcal{M}}}
% \newcommand{\model}[0]{\ensuremath{\mathcal{M}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Caligraphic Vars
\newcommand{\cS}{{\mathcal{S}}}
\newcommand{\cR}{{\mathcal{R}}}
\newcommand{\cA}{{\mathcal{A}}}
\newcommand{\cG}{{\mathcal{G}}}
\newcommand{\cE}{{\mathcal{E}}}
\newcommand{\cV}{{\mathcal{V}}}
\newcommand{\cB}{{\mathcal{B}}}
\newcommand{\cX}{{\mathcal{X}}}
\newcommand{\cH}{{\mathcal{H}}}
\newcommand{\cU}{{\mathcal{U}}}
\newcommand{\cW}{{\mathcal{W}}}
\newcommand{\cC}{{\mathcal{C}}}
\newcommand{\cO}{{\mathcal{O}}}

\newcommand{\cL}{{\mathcal{L}}}

% Bold vars
\newcommand{\ba}{{\mathbf{a}}}
\newcommand{\bff}{{\mathbf{f}}}
\newcommand{\bh}{{\mathbf{h}}}
\newcommand{\br}{{\mathbf{r}}}
\newcommand{\bs}{{\mathbf{s}}}
\newcommand{\bt}{{\mathbf{t}}}
\newcommand{\bu}{{\mathbf{u}}}
\newcommand{\bv}{{\mathbf{v}}}
\newcommand{\bw}{{\mathbf{w}}}
\newcommand{\bx}{{\mathbf{x}}}
\newcommand{\by}{{\mathbf{y}}}
\newcommand{\bz}{{\mathbf{z}}}
\newcommand{\bX}{{\mathbf{X}}}
\newcommand{\bZ}{{\mathbf{Z}}}

\newcommand{\reals}{{\mathbb{R}}}


% \mathfrak caligraphgy
\newcommand{\ff}{{\boldsymbol{\mathfrak{F}}}}
\newcommand{\fr}{{\boldsymbol{\mathfrak{r}}}}

%d'-general position

\newcommand{\Hnd}{\boldsymbol{\mathcal{H}}_{n,d}}
\newcommand{\Hndp}{\boldsymbol{\mathcal{H}}_{(n),d}}
\newcommand{\Hndo}{\boldsymbol{\mathcal{H}}_{n-1,d-1}}
\newcommand{\xnd}{\boldsymbol{\mathcal{X}}_{n,d}}
\newcommand{\xndp}{\boldsymbol{\mathcal{X}}_{n,d}^{+}}
\newcommand{\xndn}{\boldsymbol{\mathcal{X}}_{n,d}^{-}}
\newcommand{\Hndd}{\boldsymbol{\mathcal{H}}_{n,d'}^{ind}}
\newcommand{\rnd}{\boldsymbol{\fr}\parenb{\cA(\Hnd)}}
\newcommand{\regionset}{\boldsymbol{\mathfrak{R}}\parenb{\mathcal{A}(\Hnd)}}
\newcommand{\regionpair}{\boldsymbol{\mathfrak{R}}\parenb{\mathcal{A}(\boldsymbol{\mathcal{H}}_{(n),d})}}
\renewcommand{\tt}[1]{\textit{#1}}
\newcommand{\rank}[1]{\textbf{rank}\parenb{#1}}
\newcommand{\lam}{\parenb{\mathbf{\Lambda}}}
\newcommand{\boldlam}{\mathbf{\boldsymbol{\Lambda}}}
\def\mathbi#1{\textbf{\em #1}}
\newcommand{\varstackrel}[3][T]{\stackrel{\raisebox{0.5ex}{\scriptsize#2}}{#3}}

%\newcommand{\boldlam}{\textLambda}
\def\BState{\State\hskip-\ALG@thistlm}

%Data space and Hypothesis space
\newcommand{\data}{\textit{data space}}
\newcommand{\hypo}{\textit{hypothesis space}}
\newcommand{\wrt}{\mathrm{wrt}}
\newcommand{\gen}{{$d'$-\textit{relaxed general position}}}
\newcommand{\up}[1]{\Upsilon_{\mathrm{dual}}\parenb{#1}}
\newcommand{\upi}[1]{\Upsilon^{-1}_{\mathrm{dual}}\parenb{#1}}
\newcommand{\vari}[1]{\varphi^{-1}_{\mathrm{dual}}\parenb{#1}}
%\newcommand{\comment}[1]{}
%00000000000Macros for variables
\newcommand{\h}{z}
\newcommand{\dt}{x}
\newcommand{\rgn}{r}
%\newcommand{}{y}

